Modelling Agent-Skipping Attacks in Message Forwarding Protocols

Message forwarding protocols are protocols in which a chain of agents handles transmission of a message. Each agent forwards the received message to the next agent in the chain. For example, TLS middleboxes act as intermediary agents in TLS, adding functionality such as filtering or compressing data. In such protocols, an attacker may attempt to bypass one or more intermediary agents. Such an agent-skipping attack can the violate security requirements of the protocol. Using the multiset rewriting model in the symbolic setting, we construct a comprehensive framework of such path protocols. In particular, we introduce a set of security goals related to path integrity: the notion that a message faithfully travels through participants in the order intended by the initiating agent. We perform a security analysis of several such protocols, highlighting key attacks on modern protocols.

==> diagrams/equational-theory-backup.tex <==
\begin{table}[t]
    \normalsize
    \centering
    \begin{tabular}{p{1.8cm} | p{6.7cm}}
        \hline
        \multicolumn{1}{c|}{\bf Function} & \multicolumn{1}{c}{\bf Description} \\
        \hline
        \multicolumn{2}{c}{Hashing} \\
        \hline
        \multicolumn{1}{c|}{$\h/1$} & $\h(m)$ \\
        \hline
        \multicolumn{2}{c}{Pairing and projections} \\
        \hline
        \multicolumn{1}{c|}{$\langle \rangle/2$} & $\langle x, y \rangle$ \\
        \multicolumn{1}{c|}{$\fst/1$} & $\fst(\langle x, y \rangle) = x$ \\
        \multicolumn{1}{c|}{$\snd/1$} & $\snd(\langle x, y \rangle) = y$ \\
        \hline
        \multicolumn{2}{c}{Symmetric encryption and decryption} \\
        \hline
        \multicolumn{1}{c|}{$\senc/2$} & $\senc(m, k)$ \newline ($m$ is encrypted with a symmetric key $k$)\\
        \multicolumn{1}{c|}{$\sdec/2$} & $\sdec(\senc(m, k), k) = m$ \\
        \hline
        \multicolumn{2}{c}{Asymmetric encryption and decryption} \\
        \hline
        \multicolumn{1}{c|}{$\pk/1$} & $\pk(k)$ \newline (private key $k$ and its public key $\pk(k)$)\\
        \multicolumn{1}{c|}{$\aenc/2$} & $\aenc(m, \pk(k))$ \newline ($m$ is encrypted with a public key $\pk(k)$) \\
        \multicolumn{1}{c|}{$\adec/2$} & $\adec(\aenc(m, \pk(k)), k) = m$ \\
        \hline
        \multicolumn{2}{c}{Signatures} \\
        \hline
        \multicolumn{1}{c|}{$\true$} & $\true$ \\
        \multicolumn{1}{c|}{$\sign/2$} & $\sign(m, k)$ \newline ($m$ is signed with a private key $k$) \\
        \multicolumn{1}{c|}{$\verify/3$} & $\verify(\sign(m, k), m, \pk(k)) = \true$\\
        \hline
    \end{tabular}
    \caption{\label{table:equational-theory} Built-in message theories}
\end{table}

==> diagrams/equational-theory-figure.tex <==
\begin{figure*}[hbt]
\centering
\begin{align*}
% ---- Hashing
\h/1 &%
 \hspace{4ex} \text{Hashing}
\\
% ---- Pairing
\langle\ \rangle/2, \fst/1, \snd/1 &%
 \hspace{4ex}
     \text{Pairing and projections}
 \\ & \hspace{12ex}
     \fst(\langle x,y \rangle) = x
 \\ & \hspace{12ex}
     \snd(\langle x,y \rangle) = y
\\
% ---- Senc
\senc/2, \sdec/2 &%
 \hspace{4ex} \text{Symmetric encryption and decryption}
 \\ & \hspace{12ex} \sdec(\senc(m, k), k) = m
\\
% ----- Aenc
\aenc/2, \adec/2, \pk/1 &%
 \hspace{4ex} \text{Asymmetric encryption and decryption}
 \\ & \hspace{12ex} \adec(\aenc(m, \pk(k)), k) = m
\\
% ---- Signing
\sign/2, \verify/3, \true/0 &%
\hspace{4ex} \text{Signatures}
\\ & \hspace{12ex} 
     \verify(\sign(m, k), m, \pk(k)) = \true
\end{align*}
\caption{Function symbols $\Sigma$ along with
associated intuition and equational theory $E$}
\label{fig:equational-theory}
\end{figure*}

==> diagrams/lightningPossibilityProtocol.tex <==
\begin{figure*}[tb]
\begin{tcolorbox}
% ------------------------------------- %
% -------------- Key Gen -------------- %
% ------------------------------------- %
\textbf{Setup} \xdash[21em]
\begin{align*}
\hspace{0.5cm}&\makeNamedRule{ % --- NAME ---
Gen\_Ltk
}{
% --- INPUT ---
    \ruleFact{Fr}{ltk}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{!Ltk}{A, ltk} \\%
    \ruleFact{!Pk}{A, pk(ltk)}\\
    \ruleFact{Net}{pk(ltk)}
}
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\
&\makeNamedRule{ % --- NAME ---
Gen\_ShKey
}{
% --- INPUT ---
    \ruleFact{Fr}{k}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{!ShKey}{A, B, k}%
}%
\end{align*}
% ------------------------------------- %
% ----------- Construction ------------ %
% ------------------------------------- %
\textbf{Construction} \xdash[18em]
\begin{align*}
\hspace{0.5cm}&\makeNamedRule{% --- NAME --- %
Create
}{%
% --- INPUT ---
    \ruleFact{Fr}{p}, 
    \ruleFact{Fr}{e_E}\\
    \ruleFact{!ShKey}{D, E, k_{DE}}\\
    \ruleFact{!Pk}{E, pk_E}
}{% --- EVENT ---
    \ruleFact{Add}{p, E, \lbrace h(p), PH_E \rbrace_{k_{DE}}, `'}\\
    \ruleFact{StartBuild}{A, p}
}{% --- OUTPUT --- 
    \ruleFact{Build}{p, A, E, \lbrace h(p), \lbrace e_E \rbrace_{pk_E} \rbrace_{k_{DE}}}%
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\[0.8em]%
&\makeNamedRule{% --- NAME ---
Wrap
}{
% --- INPUT ---
    \ruleFact{Build}{ p, A, N, \lbrace m, PH_X \rbrace_{k_{NX}}}\\
    \ruleFact{!Pk}{ N, pk_N }, \ruleFact{Fr}{e_N}\\
    \ruleFact{!ShKey}{M, N, k_{MN}}
}{% --- EVENT ---
    \ruleFact{Add}{p, N, m, m }
}{% --- OUTPUT --- 
    \ruleFact{Build}{p, A, M, \lbrace m, PH_N \rbrace_{k_{MN}} }%
} %
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\[0.8em]
&\makeNamedRule{% --- NAME ---
Send
}{
% --- INPUT ---
    \ruleFact{Build}{p, A, M, \{ m \}_k}\\
    \ruleFact{!ShKey}{A, M, k}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{Net}{\{ m \}_k}\\%
    \ruleFact{InitState}{A, p, pkeys}
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% ------------ Forwarding ------------- %
% ------------------------------------- %
\textbf{Forwarding} \xdash[18em]
\begin{align*}
\hspace{0.5cm}& \makeNamedRule{% --- NAME ---
Unwrap
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ h(x), PH_C \}_{k_{BC}} }\\
    \ruleFact{!Ltk}{C, ltk)}\\
    \ruleFact{!ShKey}{B, C, k_{BC}}\\
    \ruleFact{!ShKey}{C, D, k_{CD}}
}{% --- EVENT ---
    \ruleFact{Forward}{C, m, m }
}{% --- OUTPUT --- 
    \ruleFact{Net}{\{ h(x), PH_D \}_{k_{CD}}}\\%
    \ruleFact{FwdState}{C, h(x), e_C, \pk(keys)}
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% --------------- Reply --------------- %
% ------------------------------------- %
\textbf{Reply} \xdash[18em]
\begin{align*}
\hspace{0.5cm}&\makeNamedRule{% --- NAME --- 
Reply
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ h(p), PH_E \}_{k_{DE}} }\\
    \ruleFact{!Ltk}{E, ltkE, pkE)}\\
    \ruleFact{!ShKey}{D, E, k_{DE}}
}{% --- EVENT ---
    \ruleFact{Forward}{E, h(p), `' }
    \ruleFact{Backward}{E, `', p }
}{% --- OUTPUT --- 
    \ruleFact{Net}{ \{ p, \sign(p, e_E) \}_{k_{DE}} }
}% 
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% --------------- Response --------------- %
% ------------------------------------- %
\textbf{Response} \xdash[18em]
\begin{align*}
\hspace{0.5cm}& \makeNamedRule{% --- NAME ---
Backward
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ p, \sign(p, keys) \}_{k_{CD}} }\\
    \ruleFact{!ShKey}{B, C, k_{BC}}\\
    \ruleFact{!ShKey}{C, D, k_{CD}}\\
    \ruleFact{FwdState}{C, h(p), e_C, pkeys}
}{% --- EVENT ---
    \ruleFact{Backward}{C, p, p }\\
    \ruleFact{Equal}{\verify(sig,p,pkeys), \true}
}{% --- OUTPUT --- 
    \ruleFact{Net}{ \{ p, \sign(p, \langle keys, e_C \rangle \}_{k_{BC}} }
}%
\\
\hspace{0.5cm}& \makeNamedRule{% --- NAME ---
Finish
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ p, sig \}_{pk} }\\
    \ruleFact{!ShKey}{A, B, k_{AB})}\\
    \ruleFact{InitState}{A, p, pkeys}
}{% --- EVENT ---
    \ruleFact{Equal}{\verify(sig,p,pkeys), \true}
}{% --- OUTPUT --- 
    \hspace{4ex}-\hspace{4ex}\ 
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
\end{tcolorbox}
    \caption{Rewriting rules for protocol shown in Figure~\ref{fig:lightning-sig-msc}. Some terms
    are compressed for space: see full definitions
    in Appendix text.
        \label{fig:lightning-possibility-protocol-rules}}
\end{figure*}

==> diagrams/pathSymmetryEquation.tex <==
\begin{tcolorbox}%
\vspace{-2ex}%
\begin{align*}%
\hspace{2ex}%
% ^ This flushes the entire environment just a little
% bit to the right, so that it's just off the text
& \forall M_i, M_j, f_i, t_j, t_i, x, y, %
\\ & \hspace{8ex} \hash tf_i, \hash tf_j, \hash tr_i, \st
\\ &
\hspace{0ex}( \not\exists \hash tc_j \st \ruleFactAtTime{Corrupt}{M_j}{tc_j})
\\ &
\hspace{0ex} \wedge \ruleFactAtTime{Forward}{M_j, x, t_j}{tf_j}
\\ &
\hspace{0ex} \wedge \big( 
\\ &
\hspace{4ex} \big( \hspace{1.5ex} \ruleFactAtTime{Forward}{M_i, f_{i}, x}{tf_i}
\\ &
\hspace{5ex} \wedge \ruleFactAtTime{Backward}{M_i, y, t_i}{tr_i}
\\ &
\hspace{4.5ex} \big) \vee \big(
% Corrupt branch
\\ & \hspace{6ex}
\exists \hash tc_i \st
\\ & \hspace{10ex}
    \ruleFactAtTime{Corrupt}{M_i}{tc_i}
\\ & \hspace{8ex}
    \wedge \ruleFactAtTime{K}{\langle f_{i}, x \rangle}{tf_i}
\\ & \hspace{8ex}
    \wedge \ruleFactAtTime{K}{\langle y, t_{i} \rangle}{tr_i}
\\ & \hspace{3ex} \big) \big)
%\\ & \hspace{3ex} \big)
\\ & 
\hspace{0ex} \wedge (\hash tf_{i} < \hash tf_{j} < \hash tr_{i})
\\ & \implies
\\ &
\exists f_j, \hash tr_j \st (\hash tf_{j} < \hash tr_{j} < \hash tr_{i})
\\ &
\hspace{2ex} \wedge \ruleFactAtTime{Backward}{M_j, f_j, y}{tr_j}%
\hspace{8cm}
% ^ This flushes the entire equation to the far left,
% avoiding the default centering of align*
\end{align*}
\end{tcolorbox}

==> diagrams/pathVerificationEquation.tex <==
\begin{figure}[h]
\begin{tcolorbox}
\vspace{-2ex}
\[{\setstretch{1.3} \begin{array}{ l}
 \forall A, M_i, M_j, p_{ID}, f_i, t_i, f_j, t_j, %
\\ \hspace{4ex} \hash ta_i, \hash ta_j, \hash tk_i, \hash ts \st
\\  
(\not\exists \hash ta_c \st \ruleFactAtTime{Corrupt}{A}{ta_c})
\\
\hspace{0ex} \wedge \ruleFactAtTime{StartBuild}{A, p_{ID}}{ts}
\\ 
\hspace{0ex} \wedge \ruleFactAtTime{Complete}{E, p_{ID}}{tf}
\\ 
\hspace{0ex} \wedge \ruleFactAtTime{Add}{p_{ID}, M_i, f_i, t_i}{ta_i}
\\
\hspace{0ex} \wedge \ruleFactAtTime{Add}{p_{ID}, M_j, f_j, t_j}{ta_j}
\\
\hspace{0ex} \wedge (\hash ts < \hash ta_i < \hash ta_j)
\\
\hspace{0ex} \wedge \big(
\ruleFactAtTime{Forward}{M_i, f_i, t_i}{tk_i} \big) 
\\
\implies
\\
\hspace{0ex} \exists \hash tk_j \st \, (\hash tk_j < \hash tk_i)
\\
\hspace{0ex} \wedge \big(
\\
\hspace{4ex} \big( \ruleFactAtTime{Forward}{M_j, f_j, t_j}{tk_j} \big)
\\
\hspace{2ex} \vee \, \big( \, \exists\  \hash tc_j \st \ruleFactAtTime{Corrupt}{M_j}{tc_j} \land
\\
\hspace{6ex} \ruleFactAtTime{K}{\langle f_j, t_j \rangle}{tk_j}  \big)
\\  \hspace{2.15ex} \, \big)%
\hspace{12cm} % <-- Extra padding to flush the array to the left
\end{array}
}\]
\end{tcolorbox}
\caption{Statement of the Verification-Dependent Path Integrity
security goal
    \label{fig:verification-dependent-path-integrity-definition}
}
\end{figure}

==> diagrams/securityGoalIntuitions.tex <==
\begin{figure}[hb]
%%\begin{figure*}[hb]
%%    \begin{subfigure}{0.43\textwidth}
%%    \includegraphics[width=\textwidth]{mscs/integrity_security_intuition_left.pdf}
%%    \caption{A partial trace.
%%    Through $\factFont{Add}$ facts, 
%%    $A$ establishes a path
%%    order such that $M_i <_\pi M_j$, and $M_j$ has
%%    forwarded the message}
%%    \end{subfigure}%
%%    \hspace{0.5em}%
%%    {\Huge $\implies$}%
%%    \hspace{1em}%
%%    \begin{subfigure}{0.43\textwidth}
%%    \includegraphics[width=\textwidth]{mscs/integrity_security_intuition_right.pdf}
%%    \caption{The security goal is satisfied only if the
%%    only way the partial trace can be realised is
%%    if $M_i$ had also forwarded the message}
%%    \end{subfigure}
%%    \caption{Intuition of the structure of the
%%    Path Integrity, Verification-Dependent Path Integrity
%%    and Path Symmetry goals}
%    \SM{``in this section'' is not specific enough for floats like this. Better to mention the security goals explicitly.}
%    \ZS{Reword}
    \caption{\HJ{Figure commented out}}
    \label{fig:security-goal-intution}
%%\end{figure*}
\end{figure}

==> diagrams/symmetricOnionProtocol.tex <==
\begin{figure*}[b]
\centering
\includegraphics[width=0.7\textwidth]{mscs/public_key_example_roundtrip.pdf}
\vspace{0ex}

\begin{tcolorbox}
% ------------------------------------- %
% -------------- Key Gen -------------- %
% ------------------------------------- %
\textbf{Setup} \xdash[21em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{ % --- NAME ---
Gen\_Ltk
}{
% --- INPUT ---
    \ruleFact{Fr}{ltk}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{!Ltk}{A, ltk}, \ 
    \ruleFact{!Pk}{A, \pk(ltk)}, \ 
    \ruleFact{Net}{\pk(ltk)}
}
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% ----------- Construction ------------ %
% ------------------------------------- %
\textbf{Construction} \xdash[18.1em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{% --- NAME --- %
Create
}{%
% --- INPUT ---
    \ruleFact{Fr}{p}\\
    \ruleFact{!Pk}{E, pkE}\\ 
    \ruleFact{!Ltk}{A, ltkA}
}{% --- EVENT ---
    \ruleFact{Add}{p, E, \{ p, E, \sign(p, ltkA) \}_{pkE}, `'}\\
    \ruleFact{StartBuild}{A, p}
}{% --- OUTPUT --- 
    \ruleFact{Build}{p, E, A, \{ p, E, \sign(p, ltkA) \}_{pkE} }%
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\[0.8em]%
&\makeNamedRule{% --- NAME ---
Wrap
}{
% --- INPUT ---
    \ruleFact{Build}{ p, M_i, A, m}\\
    \ruleFact{!Pk}{ M_{j}, \mi{pk} }
}{% --- EVENT ---
    \ruleFact{Add}{p, E, m, \{ m \}_{\mi{pk}} }
}{% --- OUTPUT --- 
    \ruleFact{Build}{p, M_{j}, A, \{ m \}_{\mi{pk}}}%
} %
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\[0.8em]
&\makeNamedRule{% --- NAME ---
Send
}{
% --- INPUT ---
    \ruleFact{Build}{p, A, M_1, m}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{Net}{m}\\%
    \ruleFact{InitState}{A, p}
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% ------------ Forwarding ------------- %
% ------------------------------------- %
\textbf{Forwarding} \xdash[18.7em]
\begin{align*}
\hspace{1cm}& \makeNamedRule{% --- NAME ---
Unwrap
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ m \}_{\pk(ltk)} }\\
    \ruleFact{!Ltk}{M_i, ltk}
}{% --- EVENT ---
    \ruleFact{Forward}{M_i, \{ m \}_{\pk(ltk)}, m }
}{% --- OUTPUT --- 
    \ruleFact{Net}{m}%
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% ------------- Receive --------------- %
% ------------------------------------- %
\textbf{Receive} \xdash[20.5em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{% --- NAME --- 
Receive
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ p, sig \}_{\pk(ltkE)} }\\
    \ruleFact{!Ltk}{E, ltkE)}\\
    \ruleFact{!Pk}{A, pkA}
}{% --- EVENT ---
    \ruleFact{Forward}{E, \{ p, sig \}_{\pk(ltkE)}, `' }\\
    \ruleFact{Equal}{\verify(sig, p, pkA), \true}
}{% --- OUTPUT --- 
    \ruleFact{Rebuild}{p, A, rt, \{f(p)\}_{pkA}}
}% 
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% ------------- Receive --------------- %
% ------------------------------------- %
\textbf{Reply} \xdash[18em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{% --- NAME --- 
Rewrap
}{
% --- INPUT ---
    \ruleFact{Rebuild}{p, A, \langle rest, B \rangle, m}\\
    \ruleFact{!Pk}{B, pkB}
}{% --- EVENT ---
}{% --- OUTPUT --- 
    \ruleFact{Rebuild}{p, A, rest , \{m\}_{pkB} }
}% 
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\
\hspace{1cm}&\makeNamedRule{% --- NAME --- 
Reply
}{
% --- INPUT ---
    \ruleFact{Rebuild}{p, A, A, m }
}{% --- EVENT ---
    \ruleFact{Backward}{E, `', m}
}{% --- OUTPUT --- 
    \ruleFact{Net}{m}
}% 
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
\textbf{Response} \xdash[18em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{% --- NAME --- 
Backward
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ m  \}_{\pk(ltk)} }\\
    \ruleFact{!Ltk}{M, ltk}
}{% --- EVENT ---
    \ruleFact{Backward}{M, \{ m \}_{\pk(ltk)}, m }
}{% --- OUTPUT --- 
    \ruleFact{Net}{m}
}% 
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\
\hspace{1cm}&\makeNamedRule{% --- NAME --- 
Finish
}{
% --- INPUT ---
    \ruleFact{Net}{ \{f(p)\}_{\pk(ltk)} }\\
    \ruleFact{!Pk}{A, ltk}\\
    \ruleFact{InitState}{A, p}
}{% --- EVENT ---
}{% --- OUTPUT --- 
    \hspace{4ex}-\hspace{4ex}\ 
}% 
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
\end{tcolorbox}
    \caption{Message sequence diagram and  rewriting rules for a protocol
    satisfying Path Symmetry using nested encryption.
        \label{fig:symmetric-onion-rules}}
\end{figure*}

==> diagrams/verificationPhaseProtocol.tex <==
\begin{figure*}[b]

\centering
\includegraphics[width=0.7\textwidth]{mscs/vdpi_protocol.pdf}
\vspace{0ex}

\begin{tcolorbox}
% ------------------------------------- %
% -------------- Key Gen -------------- %
% ------------------------------------- %
\textbf{Setup} \xdash[21em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{ % --- NAME ---
Gen\_Ltk
}{
% --- INPUT ---
    \ruleFact{Fr}{ltk}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{!Ltk}{A, ltk} \\%
    \ruleFact{!Pk}{A, \pk(ltk)}\\
    \ruleFact{Net}{\pk(ltk)}
}
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\
&\makeNamedRule{ % --- NAME ---
Gen\_ShKey
}{
% --- INPUT ---
    \ruleFact{Fr}{k}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{!ShKey}{A, B, k}%
}%
\end{align*}
% ------------------------------------- %
% ----------- Construction ------------ %
% ------------------------------------- %
\textbf{Construction} \xdash[18em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{% --- NAME --- %
Create
}{%
% --- INPUT ---
    \ruleFact{Fr}{p}\\
    \ruleFact{!Pk}{E, pk_E},
    \ruleFact{!Ltk}{A, ltk_A}\\
    \ruleFact{!ShKey}{D, E, k_{DE}}\\
}{% --- EVENT ---
    \ruleFact{Add}{p, E, sig_D, `'}\\
    \ruleFact{StartBuild}{A, p}
}{% --- OUTPUT --- 
    \ruleFact{Build}{p, A, E, sig_D \lbrace p, E, sig_A \rbrace_{k_{DE}}}%
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\[0.8em]%
&\makeNamedRule{% --- NAME ---
Wrap
}{
% --- INPUT ---
    \ruleFact{Build}{ p, A, D, lastsig, \lbrace p, rt, sig\rbrace_{k_{CD}}}\\
    \ruleFact{!ShKey}{ C, D, k_{CD} },
    \ruleFact{!ShKey}{ B, C, k_{BC} }
}{% --- EVENT ---
    \ruleFact{Add}{p, C, lastsig, sig_C }
}{% --- OUTPUT --- 
    \ruleFact{Build}{p, A, C, sig_C, \lbrace p, rt, sig\rbrace_{k_{BC}} } %
} %
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\[0.8em]
&\makeNamedRule{% --- NAME ---
Send
}{
% --- INPUT ---
    \ruleFact{Build}{p, A, B, lastsig, \{ m \}_k}
    \ruleFact{!ShKey}{A, B, k}
}{% --- EVENT ---
    \hspace{4ex}
}{% --- OUTPUT --- 
    \ruleFact{Net}{\{ m \}_k}%
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% ------------ Forwarding ------------- %
% ------------------------------------- %
\textbf{Forwarding} \xdash[18em]
\begin{align*}
\hspace{1cm}& \makeNamedRule{% --- NAME ---
Unwrap
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ p, route, sig \}_{k_{BC}} }\\
    \ruleFact{!ShKey}{B, C, k_{BC}}\\
    \ruleFact{!ShKey}{C, D, k_{CD}}\\
    \ruleFact{!Ltk}{C, ltk}
}{% --- EVENT ---
    \ruleFact{Forward}{C, sig, \sign(sig, ltk) }
}{% --- OUTPUT --- 
    \ruleFact{Net}{ \{ p, route, \sign(sig, ltk) \}_{k_{CD}} }
}
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% --------------- Receive --------------- %
% ------------------------------------- %
\textbf{Receive} \xdash[18em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{% --- NAME --- 
Receive
}{
% --- INPUT ---
    \ruleFact{Net}{ \{ p, \{ route \}_{\pk(ltk)}, sig \}_{k_{DE}} }\\
    \ruleFact{!Ltk}{E, ltk)},
    \ruleFact{!ShKey}{D, E, k_{DE} }
}{% --- EVENT ---
    \ruleFact{Forward}{E, sig, `' }
}{% --- OUTPUT --- 
    \ruleFact{Check}{E, p, route, sig}%
}% 
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
% ------------------------------------- %
% --------------- Verify --------------- %
% ------------------------------------- %
\textbf{Verification} \xdash[18em]
\begin{align*}
\hspace{1cm}&\makeNamedRule{% --- NAME --- %
Verify
}{%
% --- INPUT ---
    \ruleFact{!Pk}{D, \pk(ltk)}\\
    \ruleFact{Check}{E, p, \langle rest, D \rangle, \sign(nextSig, ltk)}
}{% --- EVENT ---
}{% --- OUTPUT --- 
    \ruleFact{Check}{E, p, rest, nextSig}%
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\\[0.8em]%
&\makeNamedRule{% --- NAME ---
Finish
}{
% --- INPUT ---
    \ruleFact{Check}{E, p, A, sig}\\
    \ruleFact{!Pk}{A, pkA}
}{% --- EVENT ---
    \ruleFact{Equal}{\verify(sig, p, pkA), \true}\\
    \ruleFact{Complete}{E, p}
}{% --- OUTPUT --- 
    \hspace{4ex}-\hspace{4ex}\ 
}%
\hspace*{12cm} % This flushes things to the left since align isn't working.
\end{align*}
\end{tcolorbox}
    \caption{Intended execution and rewriting rules for protocol
    with additional verification phase.
        \label{fig:verification-phase-protocol-rules}}
\end{figure*}

==> multisetrules.tex <==
%
% The main addition of this .sty is the environment 
% multisetrule, which will draw a diagram of a multiset
% transition rule. It takes one optional parameter, which
% can be used to determine the type of diagram drawn.
% By default, it draws an arrowed-transition graph, "table"
% draws it in lines (although there are prettier ways of doing this).
% Inside the environment, use \addprelim, \addstate, \addoutput and \mtitle
%

\RequirePackage{tikz} %% Drawing diagrams
\usetikzlibrary{positioning} % Allows place-names for node positions

\RequirePackage{amsmath}       % Standard math library

\RequirePackage{environ}       % \BODY command in custom environments
\RequirePackage{ifthen}        % Allows branching
\RequirePackage{expl3, xparse} % Used for pseudo-programming


%\usepackage{changepage} %% Had this, can't remember if it's needed (no errors are thrown, but we'll see...

%%%%%%%%%%%%% Things begin Begins %%%%%%%%%%%%%

%% multisetterm takes two arguments and turns them into a 'term' of name
%% and parameters
\newcommand{\multisetTerm}[2]{\ensuremath{\operatorname{#1}(#2)}}
\newcommand{\factName}[1]{\ensuremath{\operatorname{#1}}}
%\newcommand{\eventFactName}[1]{\ensuremath{\mathbf{*#1}}}
\newcommand{\eventFactName}[1]{\ensuremath{\operatorname{#1}\hspace{-.4ex}^\star}}

\newcommand{\ruleFact}[2]{\ensuremath{\operatorname{#1}(#2)}}
\newcommand{\ruleFactAtTime}[3]{\ensuremath{\operatorname{#1}(#2)@#3}}
\newcommand{\ruleEventFact}[2]{\ensuremath{\eventFactName{#1}(#2)}}

\NewEnviron{multisetrule}[1]
  {
  \ifthenelse{\equal{#1}{lts}}{
  \drawltsusing{\BODY} %% If the sent argument is to draw a table
                          %% Jorge's table drawing \myRule command is nicer
    }
    {
  \drawltsusing{\BODY} %% Else default to drawing a graph
    }
  }

%% To make sure that everything is done in the correct order
%% i.e. variables are cleared, then the new values are loaded,
%% then the graph is drawn, we put the environment
%% inside a wrapper
\newcommand{\drawgraphusing}[1]{
    \initializelists{}
    #1
    \drawgraph
}


\newcommand{\drawtableusing}[1]{
    \initializelists{}
    #1
    \drawtable
}

\newcommand{\drawltsusing}[1]{
    \initializelists{}
    #1
    \drawlts
}

%%%%%%%%%%%%% Swap to expl syntax %%%%%%%%%%%%%

\ExplSyntaxOn

%% addprelim takes two arguments and adds to the global sequence prelims_seq
%% The 'pretty' multiset term from both of them
%% Similar definitions for output, state
\NewDocumentCommand{\addprelim}{mm}{
\seq_gput_right:Nn \g_prelims_seq{\ruleFact{#1}{#2}}

\int_gincr:N \g_prelims_length_int
\int_gset_eq:NN \g_max_seq_int \int_max:nn {\int_max:nn {\g_prelims_length_int} {\g_states_length_int}} {\g_output_length_int}
}

\NewDocumentCommand{\addoutput}{mm}{
\seq_gput_right:Nn \g_output_seq{\ruleFact{#1}{#2}}

\int_gincr:N \g_output_length_int
\int_gset_eq:NN \g_max_seq_int \int_max:nn {\int_max:nn {\g_prelims_length_int} {\g_states_length_int}} {\g_output_length_int}
}

\NewDocumentCommand{\addstate}{mm}{
\seq_gput_right:Nn \g_states_seq{\ruleEventFact{#1}{#2}}

\int_gincr:N \g_states_length_int
\int_gset_eq:NN \g_max_seq_int \int_max:nn {\int_max:nn {\g_prelims_length_int} {\g_states_length_int}} {\g_output_length_int}
}

\NewDocumentCommand{\mtitle}{m}{
\str_gset:Nn \g_title_str {#1}
}

\int_new:N \g_prelims_length_int
\int_new:N \g_states_length_int
\int_new:N \g_output_length_int
\int_new:N \g_max_seq_int
\str_new:N \g_title_str

% initializelists takes no arguments and refreshes the local lists for a drawn graph
\NewDocumentCommand{\initializelists}{}{
\seq_gclear_new:N \g_prelims_seq
\seq_gclear_new:N \g_states_seq
\seq_gclear_new:N \g_output_seq
\str_gclear_new:N \g_title_str
\int_gzero:N \g_prelims_length_int
\int_gzero:N \g_states_length_int
\int_gzero:N \g_output_length_int
\int_gzero:N \g_max_seq_int
}

% drawgraph uses the (hopefully predefined) sequences to produce a tikz graph
\NewDocumentCommand{\drawgraph}{}{
\begin{tikzpicture}
\str_if_empty:NTF \g_title_str {} {
\node[text~width=6cm,align=center] at (0,0.5+0.2*\g_max_seq_int) {
\textbf{Rule }\; \g_title_str };
}

\seq_if_empty:NTF \g_states_seq { % If states is empty
\node[draw, text~width=3.5cm] (prelims) at (-4,0) {
\prettyprint:n \g_prelims_seq };
\node[draw, text~width=3.5cm] (outputs) at (4,0) {
\prettyprint:n \g_output_seq };
\draw[->] (prelims)  edge (outputs);
} % Else
{
\node[draw, text~width=3.5cm] (prelims) at (-4,0) {
\prettyprint:n \g_prelims_seq };
%\node[draw, text~width=3.5cm] (states) at (0,0) {
%\prettyprint:n \g_states_seq };
\node[draw, text~width=3.5cm] (outputs) at (4,0) {
\prettyprint:n \g_output_seq \hrule
%\hline
\prettyprint:n \g_states_seq };

\draw[->] (prelims) edge (outputs);
}
\end{tikzpicture}
}

% drawlts uses the (hopefully predefined) sequences to produce a Jorge-style
% labelled transition system
\NewDocumentCommand{\drawlts}{}{
\begin{equation*}
 \begin{array}{cc}
    \multicolumn{2}{c}{\thead{ \print_doubleline:n \g_prelims_seq }}
    \\ \hline
    \multirow{\g_output_length_int}{*}{\thead{ \prettyprint:n \g_output_seq  }} &
    \multirow{\g_states_length_int}{*}{\thead{ \prettyprint:n \g_states_seq }}
\end{array}{\texttt{ \g_title_str }}
\end{equation*}
}

%%%%%%%%%%%%% Helper Functions for expl %%%%%%%%%%%%%

%% doubleline takes a sequence and prints it two lines at a time
%% with a small gap between lines
\cs_new:Npn \print_doubleline:n #1
{
    \seq_if_empty:NTF #1 {} {
    \bool_gset_true:N \g_alternating_marker    
    \seq_clear_new:N \l_inputseq_seq
    \str_clear_new:N \l_firstvalue_str
    \seq_set_eq:NN \l_inputseq_seq #1
    \seq_pop:NN \l_inputseq_seq \l_firstvalue_str
    \l_firstvalue_str
    \seq_map_function:NN \l_inputseq_seq \alternatingprint:n }
}

%% alternatingprint prints either a tab or a newline, followed
%% by the string it is given
\cs_new:Npn \alternatingprint:n #1
{
    \bool_if:NTF \g_alternating_marker
        {
            \hspace{3ex} #1
            \bool_gset_false:N \g_alternating_marker
        }
        {
            \\ #1
            \bool_gset_true:N \g_alternating_marker
        }
}

%% newline takes a string and prints it, followed by a newline
\cs_new:Npn \print_newline:n #1
{
    \\ #1
}

%% prettyprint takes a sequence and prints it in a pretty way
\cs_new:Npn \prettyprint:n #1
{
    \seq_if_empty:NTF #1 {} {
    \seq_clear_new:N \l_inputseq_seq
    \str_clear_new:N \l_firstvalue_str
    \seq_set_eq:NN \l_inputseq_seq #1
    \seq_pop:NN \l_inputseq_seq \l_firstvalue_str
    \l_firstvalue_str
    \seq_map_function:NN \l_inputseq_seq \print_newline:n }
}


%% drawtable uses the (hopefully predefined) sequences to produce a beautifully arranged table
\NewDocumentCommand{\drawtable}{}{
\begin{tabular}{l}
\prettytabs:n \g_prelims_seq
\cr \hline
\seq_if_empty:NTF \g_states_seq {} {
\prettytabs:n \g_states_seq \cr }
\prettytabs:n \g_output_seq

\end{tabular}
}


%% newline takes a string and prints it, followed by a newline
\cs_new:Npn \print_newrow:n #1
{
    \cr #1
}

%% prettyprint takes a sequence and prints it in a pretty way
\cs_new:Npn \prettytabs:n #1
{
    \seq_if_empty:NTF #1 {} {
    \seq_clear_new:N \l_inputseq_seq
    \str_clear_new:N \l_firstvalue_str
    \seq_set_eq:NN \l_inputseq_seq #1
    \seq_pop:NN \l_inputseq_seq \l_firstvalue_str
    \l_firstvalue_str
    \seq_map_function:NN \l_inputseq_seq \print_newrow:n }
}

\ExplSyntaxOff

==> sections/02b-lightning.tex <==
\subsection{Lightning Network}
\label{sec:lightning}

%When it comes to payment networks,
%much thought has been put into improving their efficiency
%-- both in optimising the discovery of channels
%on the network, and in choosing an optimal path for a
%payment to travel through~\cite{lightningRoutingPrivacy,lightningRouteSelection,splitPayments}.
%Malavolta \etal\cite{lightningWormhole} describe a
%wormhole attack on the Lightning network, similar to
%those demonstrated on wireless sensor
%networks~\cite{sensorWormhole},
%and propose
%a scheme to fix it. Our model can be used to both detect
%this attack and prove resistance of their amended version
%in an automated manner, whilst their proof relies on a lengthy
%construction in the computational model. 
%Finally, while Malavolta \etal give an impossibility result
%on the existence of secure two-round payment protocols, we
%instead show that under our set of assumptions such
%protocols can indeed be constructed using only standard
%cryptographic primitives.
%The full discussion is given in Section~\ref{sec:lightning}.


% -----------------------
\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.7\textwidth]{mscs/lightning_attack_messages.pdf}
    \caption{Simplified attack on the
    Lightning payment
    forwarding protocol. Dashed lines indicate out-of-band
    communication}
    \label{fig:lightning-attack}
\end{figure*}
% -----------------------

We now look at the Lightning Network~\cite{lightning},
a second-layer protocol designed to run
on top of the Bitcoin cryptocurrency. The aim of the Lightning
Network is to increase network speeds by resolving many
transactions ``off-chain''. At its core, this is done by pairs
of agents maintaining an unpublished contract, which describes
how funds are to be allocated between them. Instead of performing
transactions on the Bitcoin ledger, the shared contract is updated to
redistribute the funds. In case of payment disputes, the contract can
be published to the blockchain for resolution.

Recent work by Bursuc and Kremer~\cite{bitcoinProof}
takes steps into modelling aspects of the
Bitcoin cryptocurrency in the symbolic setting. However,
to the best of our knowledge, no such models exist for
the Lightning Network.

First, we give
an overview of the payment forwarding protocol. We then demonstrate
a fee-skimming attack, originally discovered by
Malavolta et al.~\cite{lightningWormhole}. Next we extend their work,
by demonstrating that it is possible to build a secure two-round
payment protocol using only simple cryptographic primitives.

\mysubsect{Lightning Payment Protocol}
\label{subsec:payment-forwarding-protocol}

The Lightning Network consists of a collection of nodes which
communicate using a gossip protocol. Any pair of nodes can open a
\textit{payment channel} through a channel establishment
protocol, and may choose to broadcast this information using
the gossip network. As a result, we can consider a graph of all
active participants of the network, where two nodes are connected
by an edge if and only if there exists an open public payment channel
between them. The gossip protocol aims to give agents a complete
view of this graph, allowing them to route payments along these edges.

%There are concerns about the use of gossip protocols
%in ensuring agents have an accurate view of the network
%topology~\cite{gossipDenial}, including denial of service attacks
%intended to hide information about the structure of the
%graph.
%Similarly,
%there are some theorised denial of service attacks 
%involving interfering with specific payment
%channels~\cite{lightningGriefing}, either to disrupt the
%network or to encourage the use of other channels (for example,
%to collect the associated transaction fees).

%An attacker may be motivated
%to perform such attacks in order to coerce agents to use payment
%channels under their control, for example to claim the associated
%transaction fees.

%For the sake of convenience, we will ignore such 
%potential attacks,
We assume that all agents have perfect
information about the structure of the
payment network, that all open channels are accessible,
and that agents can freely publish to and
read from the underlying blockchain whenever desired.

The Lightning payment protocol makes use of a cryptographic
scheme named \textit{Hash Time-Locked Contracts} (HTLC).
Fundamentally, HTLCs form a promise that $A$ will
pay $B$ some amount of money if $B$ is able to produce the
preimage of a hashed value $h(x)$ within a certain time limit.
Most commonly, the value $x$ is chosen by $B$, who then
supplies $A$ with the hash as a payment invoice through some
off-band communication.
%$A$ can then be sure that
%they are paying the correct person, as only $B$
%can redeem the associated HTLC.

%An HTLC resolves either when $B$ produces such a preimage 
%(in which case the funds are transferred to $B$), or when
%the time expires (in which case the funds remain with $A$).
%Although HTLCs are designed to be resolved off-chain,
%participants can publish the contracts onto the blockchain
%in order to resolve any disputes and claim their deserved
%funds.

This scheme is central to the design of the \textit{chained
payment protocol}. Suppose $A$ wishes to send funds to some
agent $D$, with whom they do not currently have an
active payment channel. The protocol proceeds as follows:

\begin{enumerate}
    \item $D$ chooses a value $x$ and sends $h(x)$ to $A$
    \item $A$ chooses some path on the network to $D$ -- say,
    via $B$ and $C$
    \item $A$ opens a HTLC with $B$, agreeing to pay $B$ if
    $B$ can produce $x$ from $h(x)$, and including forwarding
    data to the remaining agents
    \item $B$ creates a new HTLC with $C$ with the same parameters,
    who then in turn creates a HTLC with $D$
    \item $D$ is able to reproduce $x$ (as they are the one who chose
    it), and provides evidence of this to $C$, closing the HTLC and
    claiming the funds
    \item $C$ now also knows $x$, and so can claim the funds from $B$,
    who can in turn claim them from $A$
\end{enumerate}

The ability of agents to ``share'' their payment channels to other
members of the system is a key design feature of the lightning network.
Generally, this is assumed to come with \textit{fees} for using the channel -
in particular, if $A$ wishes to send $D$ an amount of money $m$, they will
instead initiate the protocol with some funds $m+t$, and each intermediate
agent claims some small share of the transmitted funds as a transaction fee.
Note that funds are committed during the
first round of the protocol (the `locking' phase), but are
not distributed until the second round (the `release' phase).

In order to provide anonymity, the lightning payment protocol uses a variant of
the Sphinx~\cite{sphinx} mix protocol. Per-hop data is generated through repeated
encryption, containing information about the route and transaction fees for each
intermediate agent. However, the hash (and its later preimage) are communicated
through HTLC establishment subprotocols on the payment channels.
As such, forwarding agents may not know the full path of the message, but have a
vested interest in the path being preserved. If they lock their funds in the
first round of the protocol, they wish to be assured that they will be rewarded
their share of the transaction fees if the payment eventually completes. This
can be expressed informally as such:
\begin{defn}{Path Symmetry (Notion)}
\label{def:path-symmetry-idea}

    If an agent forwards a message in the first round of a symmetric
    path protocol, the protocol should not be able to complete without
    them also forwarding the message on the return journey.
\end{defn}
Unfortunately, the Lightning Network chained payment protocol also exhibits a skipping attack.
It is detailed by Malavolta \etal\cite{lightningWormhole}. Unlike in the previous subsection,
this attack arises on the return trip of the message, when the hash pre-image is sent back
along the original path in order to resolve the HTLCs.
Here, a corrupt agent $M_i$ sends a
non-adjacent agent $M_j$ the hash preimage $x$ through an off-band channel.
Although $M_i$ loses funds (the HTLC against them
is redeemed but they do not turn in $x$ to the next agent in the chain),
$M_j$ gains the same amount, as no-one can redeem the HTLC against
$M_j$. Further, $M_j$ also gains the transaction fees of every agent
in between the two corrupt agents. The net result is that
$M_i$ and $M_j$ skim the transaction fees of the other agents on the
path.
These agents may not be aware the attack has even taken place,
instead assuming that the payment failed, allowing the associated HTLCs to time out.

Figure~\ref{fig:lightning-attack} contains a simplified diagram of the skipping attack on the
lightning payment protocol. Note that we abstract the instantiation and later resolution of HTLCs
into individual messages. We do not include the information stored in per-hop packets, which
enable the agents to know who to route the message to.

\mysubsect{`Wormhole'-Free Payment Protocols Do Exist}
\label{subsec:impossibility-result}

In addition to demonstrating this attack and designing a new cryptographic
primitive (named an Anonymous Multi-Hop Lock), which is used to amend
the protocol, Malavolta \etal prove `wormholes' cannot be avoided.
More specifically:

\begin{thm}{(Malavolta \etal \cite[Theorem 1]{lightningWormhole})}\label{thm:malavolta-impossibility}
    
    For all two-round (without broadcast channels) multi-hop payment
    protocols there exists a path prone to the wormhole attack.
    
\end{thm}

Here, ``round'' refers to interactions between
adjacent agents. Thus, a round-trip is considered to be two
``rounds'': one for the forward trip and one for the return trip.

The model used in this paper differs in several aspects from that of
Malavolta \etal (the full
model, along with a more formal expression of this
result, labelled Theorem 5, is in their paper~\cite{lightningWormhole}).

The most significant difference relates to agents'
knowledge of the path -- in their model the only starting knowledge is
the hashed value $h(x)$ shared between the two endpoints, and
encryption keys shared between adjacent agents on the network.
However, the gossip protocol underlying the Lightning Network
aims to ensure that the network topology is public knowledge.
This gossip network broadcasts information about open payment
channels, their status, as well as agent identities and their
public keys.

By extending the starting knowledge with this information,
we instead have the following result:

\begin{thm}{(Possibility)}
\label{thm:malavolta-possibility}

	There exists a payment protocol with one round trip
	which does not admit a wormhole attack.
\end{thm}
We discuss this in more detail in Section~\ref{sec:path-integrity},
after formally introducing our security goals. Intuitively, if the
initiating agent has knowledge of the path at the start of the protocol,
they are able to construct per-hop packets for each participant that
include the necessary information to construct a chain of MACs that is
verified by each agent in turn. Indeed, the wormhole-free protocol proposed
by Malavolta~\etal uses an additional round of communication
to establish a set of terms used for a similar purpose (but using a
bespoke cryptographic primitive).
%They prove
%the security of their protocol using a game-hopping
%proof in the computational model.

Our framework can be used to identify the attack on the Lightning network,
as a violation of (a formal version of) the Path Symmetry goal above.
We emphasise two key contributions from our approach
over the prior work of Malavolta~\etal:
\begin{itemize}
    \item We prove that \textit{no additional
    round trips} are needed to avoid wormhole
    attacks on payment networks
    \item We demonstrate that \textit{no additional
    cryptographic primitives} are needed to achieve
    this security
\end{itemize}

%Our models for the Lightning Network are built from the
%Lightning ``Bolt'' specification\cite{lightingBoltSpecification}, which is a continually-updated
%document. We model communication between pairs of agents using
%symmetric encryption, with per-hop payloads encrypted using
%nested asymmetric encryption. The endpoint is assumed to be able
%
